Lower Bounds on $0$-Extension with Steiner Nodes

In the $0$-Extension problem, we are given an edge-weighted graph $G=(V,E,c)$, a set $T\subseteq V$ of its vertices called terminals, and a semi-metric $D$ over $T$, and the goal is to find an assignment $f$ of each non-terminal vertex to a terminal, minimizing the sum, over all edges $(u,v)\in E$, the product of the edge weight $c(u,v)$ and the distance $D(f(u),f(v))$ between the terminals that $u,v$ are mapped to. Current best approximation algorithms on $0$-Extension are based on rounding a linear programming relaxation called the \emph{semi-metric LP relaxation}. The integrality gap of this LP, with best upper bound $O(\log |T|/\log\log |T|)$ and best lower bound $\Omega((\log |T|)^{2/3})$, has been shown to be closely related to the best quality of cut and flow vertex sparsifiers. We study a variant of the $0$-Extension problem where Steiner vertices are allowed. Specifically, we focus on the integrality gap of the same semi-metric LP relaxation to this new problem. Following from previous work, this new integrality gap turns out to be closely related to the quality achievable by cut/flow vertex sparsifiers with Steiner nodes, a major open problem in graph compression. Our main result is that the new integrality gap stays superconstant $\Omega(\log\log |T|)$ even if we allow a super-linear $O(|T|\log^{1-\varepsilon}|T|)$ number of Steiner nodes.

==> 0_ext_upper.tex <==
\newcommand{\Poly}{\mathcal{P}}
\newcommand{\TS}{\mathcal{T}}

\section{Upper Bound}
In this section, we prove that for any $\zesn$ instance, there is a solution of size only depending on $k$ such that achieves stretch at most $1$.

We use the metric space defined by the tight span defined by the distance between the terminals. Consider the $k$-dimensional vector space, we define the polytope $\Poly(T)$ to be the set of vecotrs $x$ such that for any $i$ and $j$, $x_i+x_j \ge \ell(t_i,t_j)$. The tight span $\TS(T)$ is the set of vectors $x \in \Poly(T)$ such that for any $i$, there exists a $j$ such that $x_i+x_j = \ell(t_i,t_j)$. The tight span metric space is the metric whose point set is $\TS(T)$, and the distance between two points $x$ and $y$ is defined by the $\ell_{\infty}$ norm $\norm{x-y}_{\infty}$. For any terminal $t_i$, we define the vector represent it as $x^{t_i} = (\ell(t_1,t_i),\ell(t_2,t_i),\dots,\ell(t_k,t_i))$. The following claim shows that for any vector $x$, $x_i$ is the distance between $x$ and $t_i$.

\begin{claim} 
    For any $x$ in the metric space, $\norm{x^{t_i} - x}_{\infty} = x_i$.
\end{claim}

\begin{proof}
    For any $j \neq i$, $x_i+x_j\ge \ell(t_i,t_j)$ by triangle inequality, so $x^{t_i}_j-x_j \le x_i$. Furthermore, by minimality, there exists an index $j'$ such that $x_j+x_{j'} = \ell(t_j,t_{j'})$. We have 
    $$x_j -x^{t_i}_j = \ell(t_j,t_{j'}) - x_{j'} - \ell(t_i,t_j) \le \ell(t_i,t_{j'}) - x_{j'} \le x_i$$
    by triangle inequality. Therefore, $\card{x^{t_i}_j-x_j} \le x_i$ for any $j \neq i$ and $\card{x^{t_i}_i-x_i} = x_i$, which means $\norm{x^{t_i} - x}_{\infty} = x_i$.
\end{proof}

We first project each vertex in graph to the tight span metric $\TS(T)$, and prove that the distance between each pair of vertex will only decrease; and then we define a set of steiner nodes and give a random scheme that project each point in the metric space to the steiner nodes such that any two points in the metric space will keep their distance in expectation.

\subsection{Projection of the Points}
In this section, we project each point in the graph to the metric space. Given a point $v$, suppose the distances between $v$ and each terminal are $d_1,d_2,\dots,d_k$. We construct the projection point $x=f(v)$ by the following algorithm that is a generalization of the project algorithm in the proof of \Cref{lem:embed-tree}. Roughly speaking, we keep decreasing each $d_i$ at the same rate, and whenever a triangle inequality is tight, we stop decreasing the corresponding $d_i$.

\begin{algorithm}[H]\label{alg:project}
\caption{Project a point to the metric}
\SetAlgoLined
$S \leftarrow [k]$.\;
\While{$S \neq \emptyset$}
{
    For any $i,j \in S$, $\Delta_{i,j} \leftarrow (d_i+d_j-\delta(t_i,t_j))/2$.\;
    For any $i\in S$ and $j \notin S$, $\Delta_{i,j} \leftarrow d_i+x_j-\delta(t_i,t_j)$.\;
    For any $i \in S$, $\Delta_i \leftarrow \min_j\{\Delta_{i,j}\}$.\;
    $\Delta \leftarrow \min_{i\in S} \Delta_i$.\;
    \For{$i$ such that $\Delta_i = \Delta$}{
        $x_i \leftarrow d_i - \Delta$.\;
        $S \leftarrow S - i$.\;
    }
}
Return $x=(x_1,x_2,\dots,x_k)$.\;
\end{algorithm}

We first prove the following property of the projection.    

\begin{claim} \label{clm:project}
For any index $i$, there is an index $j$ such that $x_i+x_j = \delta(t_i,t_j)$ and $d_i-x_i \ge d_j-x_j$.
\end{claim}

\begin{proof}
When an index $i$ is removed from $S$ and $x_i$ is fixed, we have $d_i-x_i = \Delta = \Delta_i \le \Delta_{i,j}$ for any $j$. Thus, for any index $j$ inside $S$ after this iteration, $\Delta_{i,j}$ will only increase. Thus for any $i$ and $j$, $\Delta_{i,j}$ does not decrease in each iteration, and so are $\Delta_i$ and $\Delta$.

For any index $i$, consider the iteration that $x_i$ is fixed, we have an index $j$ such that $\Delta_{i,j} = \Delta = d_i-x_i$. If $j \in S$, then $\Delta \le \Delta_j \le \Delta_{i,j} \le \Delta$, and thus $\Delta_j = \Delta$, which menas $x_j$ is also fixed in the same iteration, and so $d_i-x_i = \Delta_{i,j} = d_j-x_j$ and $x_i+x_j = d_i+d_j - 2\Delta_{i,j} = \delta(t_i,t_j)$. If $j \notin S$, then $x_i + x_j = d_i - \Delta_{i,j} + x_j = \delta(t_i,t_j)$. Furthermore, since $x_j$ is fixed before this iteration, we have $d_i-x_i = \Delta \ge d_j-x_j$ since $\Delta$ is not decreasing in each iteration.
\end{proof}

Now we prove that after projection, the distance between two point will not increase.

\begin{lemma} \label{lem:proj_dis}
    For any two vertex $u,v$ in the graph, suppose $x=f(u)$ and $y=f(v)$, $\norm{x-y}_{\infty} \le \ell(u,v)$.
\end{lemma}

\begin{proof}
    For any $i$, define $\Delta^u_i$ and $\Delta^v_i$ as $\ell(u,t_i) - x_i$ and $\ell(v,t_i) - y_i$. By definition of $\ell_{\infty}$ norm and symmetry, it is sufficient to prove that for any $i$, $x_i-y_i \le \ell(u,v)$. By definition, 
    $$x_i-y_i = (\ell(u,t_1) - \Delta^u_i) - (\ell(v,t_1) - \Delta^v_i) \le \ell(u,v) - \Delta^u_i + \Delta^v_i.$$ 
    By \Cref{clm:project}, there is an index $j$ such that $x_i+x_j = \ell(t_i,t_j)$ and $\Delta^u_i \ge \Delta^u_j$. We have 
    $$x_i-y_i \le (\ell(t_i,t_j) - x_j) - (\ell(t_i,t_j) - y_j) = y_j - x_j.$$
    and 
    $$
    y_j - x_j \le \ell(u,v) - \Delta^v_j + \Delta^u_j \le \ell(u,v) - \Delta^v_j + \Delta^u_i.
    $$
    If $\Delta^v_i \le \Delta^v_j$, we have $2(x_i-y_i) \le 2\ell(u,v) - \Delta^v_j + \Delta^v_i \le 2\ell(u,v)$. If $\Delta^v_i > \Delta^v_j$, the index $j$ satisfies $\Delta^u_i \ge \Delta^u_j$, $\Delta^v_i > \Delta^v_j$ and $x_i-y_i \le y_j-x_j$. 

    By the same analysis, regarding $y_j-x_j$, we can either prove $y_j-x_j \le \ell(u,v)$ or there exists an index $i'$ such that $\Delta^v_i > \Delta^v_j \ge \Delta^v_{i'}$, $\Delta^u_i \ge \Delta^u_j > \Delta^u_{i'}$ and $x_i-y_i \le y_j-x_j \le x_{i'}-y_{i'}$. And in the later case, we can continue using the same analysis on $x_{j'}-y_{j'}$. If we keep doing the same analysis, we either prove $x_i - y_i \le \ell(u,v)$ or construct an infinite list of index $i_1,i_2,\dots$ such that for any $p$, $\Delta^u_{i_p}>\Delta^u_{i_{p+1}}$ and $\Delta^v_{i_p}>\Delta^v_{i_{p+1}}$, which is not possible. 
\end{proof}

\subsection{Project the Points in Tight Span to the Steiner Nodes}
In this section, we define the steiner nodes. For any vector $x$ in the tight span $\TS(T)$, define $\Gamma(x)$ as the graph whose vertex set is $[k]$, and two vertex $i$ and $j$ is connected if $x_i+x_j = \ell(t_i,t_j)$. We say the vector $x$ is an extreme point if $\Gamma(x)$ is connected and not bipartite. It is clear that any two extreme point $x$ and $y$ has different $\Gamma(x)$ and $\Gamma(y)$. Therefore, there are finite number of extreme points. 



==> headers.tex <==
\iffalse
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{patterns}
\usetikzlibrary{calc}
\usetikzlibrary{fit}
\usetikzlibrary{snakes}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{petri,decorations.markings}
\fi

\renewcommand{\top}{T}

\RequirePackage{silence}
\WarningFilter{remreset}{The remreset package}
\usepackage{fancybox}
\usepackage{enumitem}

\setlistdepth{9}

\newlist{myEnumerate}{enumerate}{5}
\setlist[myEnumerate,1]{label=\arabic*.}
\setlist[myEnumerate,2]{label=(\alph*)}
\setlist[myEnumerate,3]{label=\roman*.}
\setlist[myEnumerate,4]{label=\Alph*.}
\setlist[myEnumerate,5]{label=\Roman*.}
%\setlist[myEnumerate,6]{label=(\arabic*)}
%\setlist[myEnumerate,7]{label=(\Roman*)}
%\setlist[myEnumerate,8]{label=(\Alph*)}
%\setlist[myEnumerate,9]{label=(\roman*)}

%\usepackage{kbordermatrix}
%\renewcommand{\kbldelim}{(}% Left delimiter
%\renewcommand{\kbrdelim}{)}% Right delimiter
\usepackage{blkarray}
\usepackage{array}
%\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{x}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand{\mLabel}[1]{\mbox{$\scriptstyle{#1}$}}

\usepackage{stackengine}
\newcommand\xrowht[2][0]{\addstackgap[.5\dimexpr#2\relax]{\vphantom{#1}}}
%\usepackage{enumerate}

\newcommand{\gy}{G_{\sigma_n}^{\mathrm{yes}}}
\newcommand{\gn}{G_{\sigma_n}^{\mathrm{no}}}
\newcommand{\dtv}{D_{\mathrm{TV}}}

\usepackage{amsmath,amsfonts,amssymb,amsthm,bm}
\usepackage{color,xcolor}
%\usepackage[colorlinks=true]{hyperref}
\usepackage{nameref}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\definecolor{myred}{rgb}{0.8,0.25,0.25}
\definecolor{DarkRed}{rgb}{0.7, 0.0, 0.0}
\usepackage[linktocpage=true, pagebackref=true,colorlinks, linkcolor=DarkRed,citecolor=ForestGreen, bookmarks,bookmarksopen,bookmarksnumbered]{hyperref}

\usepackage[noabbrev,nameinlink]{cleveref}
\crefname{property}{property}{Property}
\creflabelformat{property}{(#1)#2#3}
\crefname{equation}{eq}{Eq}
\creflabelformat{equation}{(#1)#2#3}
\usepackage[procnumbered,ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{amsfonts}
\usepackage{thm-restate}
\usepackage{blindtext}
\usepackage{thm-restate}

\iffalse
\textheight 8.5in
\topmargin -0.2in
\oddsidemargin 0.20in
\textwidth 6.3in
\fi

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemm}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{warning}[theorem]{Warning}

\theoremstyle{definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[lemm]{Assumption}
\newtheorem{definition}[lemm]{Definition}
\newtheorem{remark}[lemm]{Remark}
\newtheorem{problem}{Problem}


\newcommand{\highlight}[1]{\colorbox{yellow}{#1}}


\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

\newenvironment{algbox}[0]{%\vskip 0.2in
\noindent
%\begin{figure}
  \begin{center}
\begin{fminipage}{1\textwidth}%{6.3in}
}{
\end{fminipage}
\end{center}
%\end{figure}
%\vskip 0.2in
}

%\newenvironment{probbox}[0]{\vskip 0.1in
%%\noindent 
%  \begin{center}
%        \begin{fminipage}{5.7in}
%}{
%\end{fminipage}
%\end{center}
%\vskip 0.1in
%}

% Algorithm2e
\DontPrintSemicolon
\SetKw{KwAnd}{and}
\SetProcNameSty{textsc}
\SetFuncSty{textsc}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\def\dr{\mathrm{d}}

\def\pleq{\preceq} %curlyeq}
\def\pgeq{\succeq} %curlyeq}
\def\pge{\succ}
\def\ple{\prec}
\def\sc{\textsc{SC}}

\newcommand\AGM{\textsc{UnweightedCutSparsify}}
\newcommand\WGM{\textsc{WeightedCutSparsify}}
\newcommand\WL{\textsc{WeightedEdgeSampler}}

\newcommand\HVS{\textsc{HeavyEdgeSketch}}
\newcommand\HVR{\textsc{HeavyEdgeRecovery}}

\newcommand\WSS{\textsc{SpectralSketch}}
\newcommand\WSR{\textsc{SpectralRecovery}}

\newcommand\SQS{\textsc{SquareSketch}}
\newcommand\SQR{\textsc{SquareRecovery}}

\newcommand\SVS{\textsc{SquareHeavySketch}}
\newcommand\SVR{\textsc{SquareHeavyRecovery}}

\newcommand\SSQ{S^{\mathrm{sq}}}
\newcommand\SSS{S^{\mathrm{ss}}}
\newcommand\SHV{S^{\mathrm{hv}}}
\newcommand\SSV{S^{\mathrm{sqh}}}

\def\detp{\det\nolimits_{+}}
\def\detb#1{\det\nolimits_{#1}}
\def\detz{\det\nolimits_{(0,\zeta]}}
\def\detzz{\det\nolimits_{(0,\zeta']}}
\def\detl{\det\nolimits_{\ell}}
\def\detll{\det\nolimits_{\ell'}}
\def\detn{\det\nolimits}

\def\dr{\mathrm{d}}

\def\Approx#1{\approx_{#1}}

\def\Span#1{\textbf{Span}\left(#1  \right)}
\def\bvec#1{{\mbox{\boldmath $#1$}}}


\def\prob#1#2{\mathrm{Pr}_{#1}\left[ #2 \right]}
\def\pr#1{\mathrm{Pr}\left[ #1 \right]}
\def\pvec#1#2{\vec{\mbox{P}}^{#1}\left[ #2 \right]}
\def\expec#1#2{{\mathbb{E}}_{#1}\left[ #2 \right]}
\def\ex#1{{\mathbb{E}}\left[ #1 \right]}
\def\var#1{\mbox{\bf Var}\left[ #1 \right]}
\newcommand{\E}{\mbox{{\bf E}}}

\def\defeq{\stackrel{\mathrm{def}}{=}}
\def\setof#1{\left\{#1  \right\}}
\def\sizeof#1{\left|#1  \right|}
\def\card#1{\left| #1 \right|}
\def\deg{\textrm{deg}}




\def\floor#1{\left\lfloor #1 \right\rfloor}
\def\ceil#1{\left\lceil #1 \right\rceil}

\def\dim#1{\mathrm{dim} (#1)}
\def\sgn#1{\mathrm{sgn} (#1)}

\def\union{\cup}
\def\intersect{\cap}
\def\Union{\bigcup}
\def\Intersect{\bigcap}

\def\eps{\epsilon}

\def\abs#1{\left|#1  \right|}

\def\rank#1{\mathrm{rank} \left(#1 \right)}
\def\trace#1{\mathrm{Tr} \left(#1 \right)}
\def\norm#1{\left\| #1 \right\|}
\def\normm#1{\lambdamax\kh{#1}}
\def\smallnorm#1{\| #1 \|}

\def\comp#1{#1^\complement}

\def\Acal{\mathcal{A}}
\def\Ncal{\mathcal{N}}
\def\Rcal{\mathcal{R}}
\def\Bcal{\mathcal{B}}
\def\Ccal{\mathcal{C}}
\def\Dcal{\mathcal{D}}
\def\Ecal{\mathcal{E}}
\def\Fcal{\mathcal{F}}
\def\Mcal{\mathcal{M}}
\def\Xcal{\mathcal{X}}
\def\Ftil{\tilde{F}}
\def\Htil{\tilde{H}}
\def\Ztil{\tilde{Z}}
\def\Ltil{\tilde{L}}
\def\wtil{\tilde{w}}
\def\Fcaltil{\tilde{\mathcal{F}}}
\def\Lambdatil{\tilde{\Lambda}}
\def\Hcal{\mathcal{H}}
\def\Ical{\mathcal{I}}
\def\Itil{\tilde{{I}}}
\def\Gcal{\mathcal{G}}
\def\Rcal{\mathcal{R}}
\def\phitil{\tilde{\phi}}
\def\Ucal{\mathcal{U}}
\def\Vcal{\mathcal{V}}
\def\Lcal{\mathcal{L}}
\def\Scal{\mathcal{S}}
\newcommand\Tcal{\mathcal{T}}
%\newcommand\Ucal{\mathcal{U}}
\newcommand\Pcal{\mathcal{P}}

\newcommand\xtil{\tilde{x}}
\newcommand\Gtil{\tilde{G}}

\newcommand\pth{\mathfrak{p}}


\newcommand\Ppsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\PPsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\ppsi{\boldsymbol{\mathit{\psi}}}
\newcommand\pphi{\boldsymbol{\mathit{\phi}}}
\newcommand\Llambda{\boldsymbol{\mathit{\Lambda}}}
\newcommand\PPi{\boldsymbol{\Pi}}

%\newcommand\ppi{\boldsymbol{\pi}}
\newcommand\ppi{\vec{\pi}}
\newcommand\cchi{\boldsymbol{\chi}}
\newcommand\aalpha{\boldsymbol{\alpha}}
\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\ggamma{\boldsymbol{\gamma}}
\newcommand\ddelta{\boldsymbol{\delta}}

\newcommand\er{R_{\mathrm{eff}}}
\newcommand\ccc{C_{\mathrm{CC}}}
\newcommand\ci{C_{\mathrm{I}}}


\def\lev{\mathtt{lev}}
\def\aa{\pmb{\mathit{a}}}
\newcommand\bb{\boldsymbol{\mathit{b}}}
%\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\dd{\boldsymbol{\mathit{d}}}
\newcommand\ee{\boldsymbol{\mathit{e}}}
\newcommand\ff{\boldsymbol{\mathit{f}}}
%\renewcommand\gg{\boldsymbol{\mathit{g}}}
\newcommand\ii{\boldsymbol{\mathit{i}}}
\newcommand\jj{\boldsymbol{\mathit{j}}}
\newcommand\kk{\boldsymbol{\mathit{k}}}
%\renewcommand\ll{\boldsymbol{\mathit{\ell}}}
\newcommand\pp{\boldsymbol{\mathit{p}}}
\newcommand{\ttau}{{\boldsymbol{\mathit{\tau}}}}
\newcommand\qq{\boldsymbol{\mathit{q}}}
\newcommand\bs{\boldsymbol{\mathit{s}}}
%\newcommand\nn{\boldsymbol{\mathit{n}}}
\newcommand\nn{\vec{n}}
\newcommand\mm{\vec{m}}
\newcommand\rr{\boldsymbol{\mathit{r}}}
\newcommand\rrh{{\boldsymbol{\widehat{\mathit{{r}}}}}}
\renewcommand\dh{\widehat{d}}
\newcommand\wh{\widehat{w}}
\renewcommand\ss{\boldsymbol{\mathit{s}}}
\def\tt{\boldsymbol{\mathit{t}}}
\newcommand\uu{\boldsymbol{\mathit{u}}}
\newcommand\vv{\boldsymbol{\mathit{v}}}
\newcommand\ww{\boldsymbol{\mathit{w}}}
\newcommand\yy{\boldsymbol{\mathit{y}}}
\newcommand\zz{\boldsymbol{\mathit{z}}}
\newcommand\xx{\boldsymbol{\mathit{x}}}
\newcommand\xxbar{\overline{\boldsymbol{\mathit{x}}}}

\newcommand\dbar{d_{\mathrm{avg}}}

\renewcommand\AA{\boldsymbol{\mathit{A}}}
\newcommand\BB{\boldsymbol{\mathit{B}}}
\newcommand\CC{\boldsymbol{\mathit{C}}}
\newcommand\DD{\boldsymbol{\mathit{D}}}
\newcommand\EE{\boldsymbol{\mathit{E}}}
\newcommand\GG{\boldsymbol{\mathit{G}}}
\newcommand\II{\boldsymbol{\mathit{I}}}
\newcommand\JJ{\boldsymbol{\mathit{J}}}
\newcommand\KK{\boldsymbol{\mathit{K}}}
\newcommand\NN{\boldsymbol{\mathit{N}}}
\newcommand\MM{\mathrm{\textsf{M}}}
\newcommand\LL{\boldsymbol{\mathit{L}}}
\newcommand\HH{\boldsymbol{\mathit{H}}}
\newcommand\PP{\boldsymbol{\mathit{P}}}
\newcommand\QQ{\boldsymbol{\mathit{Q}}}
\newcommand\RR{\boldsymbol{\mathit{R}}}
\renewcommand\SS{\boldsymbol{\mathit{S}}}
\newcommand\TT{\boldsymbol{\mathit{T}}}
\newcommand\UU{\boldsymbol{\mathit{U}}}
\newcommand\WW{\boldsymbol{\mathit{W}}}
\newcommand\VV{\boldsymbol{\mathit{V}}}
\newcommand\XX{\boldsymbol{\mathit{X}}}
\newcommand\YY{\boldsymbol{\mathit{Y}}}

\def\sfy{{\sf Yes} }
\def\sfn{{\sf No} }
\newcommand\nnz{\mathrm{nnz}}
\newcommand\tv{\mathrm{TV}}
\newcommand\yes{\mathrm{yes}} % {\mathrm{yes}}
\newcommand\no{\mathrm{no}}

\newcommand\shat{\hat{s}}
\newcommand\ftil{\tilde{f}}
\newcommand\lambdatil{\tilde{\lambda}}
\newcommand\Ntil{\tilde{N}}
\newcommand\dtil{\tilde{d}}
\newcommand\Dtil{\tilde{D}}
\newcommand\MMtil{\boldsymbol{\mathit{\tilde{M}}}}
\newcommand\AAtilde{\boldsymbol{\mathit{\tilde{A}}}}
\newcommand\LLtil{\boldsymbol{\mathit{\tilde{L}}}}
\newcommand\MMtilde{\boldsymbol{\mathit{\tilde{M}}}}

\newcommand\AAn{\boldsymbol{\mathcal{A}}}
\newcommand\ZZ{\boldsymbol{\mathit{Z}}}

\newcommand\ZZtil{\widetilde{\boldsymbol{\mathit{Z}}}}

\newcommand\AAhat{\boldsymbol{\widehat{\mathit{A}}}}
\newcommand\AAapprox{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDhat{\boldsymbol{\widehat{\mathit{D}}}}
\newcommand\DDapprox{\boldsymbol{\widetilde{\mathit{D}}}}
\newcommand\LLhat{\boldsymbol{\widehat{\mathit{L}}}}
\newcommand\LLapprox{\boldsymbol{\widetilde{\mathit{L}}}}
\newcommand\MMhat{\boldsymbol{\widehat{\mathit{M}}}}
\newcommand\MMapprox{\boldsymbol{\widetilde{\mathit{M}}}}
\newcommand\ZZhat{\boldsymbol{\widehat{\mathit{Z}}}}

\newcommand\AAtil{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDtil{\boldsymbol{\widetilde{\mathit{D}}}}


\newcommand\bbtil{\boldsymbol{\tilde{\mathit{b}}}}
\newcommand\xxtil{\boldsymbol{\tilde{\mathit{x}}}}


\newcommand\Otil{\tilde{O}}
\newcommand\otil{\tilde{o}}
\newcommand\Ktil{\tilde{K}}
\newcommand\Thetatil{\tilde{\Theta}}
\newcommand\Omegatil{\tilde{\Omega}}

\newcommand\xhat{\boldsymbol{\hat{\mathit{x}}}}
\newcommand\uhat{{\hat{{u}}}}
\newcommand\vhat{{\hat{{v}}}}
\newcommand\what{{\hat{{w}}}}

\newcommand\fbf{\mathbf{f}}

\newcommand\Ghat{{\widehat{{G}}}}

\newcommand{\sym}[1]{\mathrm{sym} (#1)}

\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\diag}{\textsc{diag}}
\newcommand\LLs{\boldsymbol{\mathit{L}_s}}
\newcommand\SSi{\boldsymbol{\Sigma}}

\newcommand\dila{\mathtt{dila}}
\newcommand\cont{\mathtt{ctrc}}
\newcommand\area{\mathtt{area}}
\newcommand\vol{\mathsf{cost}}
\newcommand\scolon{\hspace{-2.5pt}:\hspace{-1.5pt}}

\newcommand\DS{\textsc{DetScheduling}}
\newcommand\DP{\textsc{DPScheduling}}
\newcommand\RI{\textsc{Rounded}}
\newcommand\PTAS{\textsc{PoiScheduling}}
\newcommand\ILP{\textsc{ILPScheduling}}
\newcommand\IP{\textsc{ILP}}
\newcommand\CHEBY{\textsc{ChebySolve}}
\newcommand\HARGD{\textsc{AlmostRegularDecomp}}
\newcommand\HED{\textsc{ExpanderDecomp}}
\newcommand\WAM{\textsc{Whack-a-mole-I}}
\newcommand\WTM{\textsc{Whack-a-mole-II}}
\newcommand\WAME{\textsc{Whack-a-mole-Exp}}

\newcommand\la{\leftarrow}

\newcommand\TEST{\textsc{Traps?}}
\newcommand\MBSWB{\textsc{NoisyBinarySearchRW}}

\newcommand\IR{\textsc{Sparisfy}}
\newcommand\SP{\textsc{SampleWR}}

\newcommand\SC{\mathrm{SC}}
\newcommand\SCN{\mathrm{SC}_n}

\newcommand{\sd}{\geq_{\mathrm{sd}}}

\newcommand{\todo}[1]{{\bf \color{red} TODO: #1}}
\newcommand{\hl}[1]{{\bf \color{orange} Huan: #1}}
%\newcommand{\yhy}[1]{{\color{blue} #1}}
%\newcommand{\zzz}[1]{{\bf \color{green} Zhongzhi: #1}}
%\newcommand{\sep}[1]{{\color{blue}#1}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\poi}[1]{\mathrm{Poi}\left(#1\right)}

\newcommand{\kh}[1]{\left(#1\right)}

\newcommand{\ip}[2]{\left\langle#1,#2\right\rangle}

\newcommand{\wmax}{w_{\max}}
\newcommand{\wmin}{w_{\min}}

\newcommand{\lambdamin}{\lambda_{\mathrm{min}}}
\newcommand{\lambdamax}{\lambda_{\mathrm{max}}}

\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\ade}[1]{{\color{blue}#1}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\by}{\mathbf{y}}

\newcommand{\dmin}{d_{\mathrm{min}}}

